SecVulEval: Benchmarking LLMs for Real-World C/C++ Vulnerability Detection

Large Language Models (LLMs) have shown promise in software engineering tasks, but evaluating their effectiveness in vulnerability detection is challenging due to the lack of high-quality datasets. Most existing datasets are limited to function-level labels, ignoring finer-grained vulnerability patterns and crucial contextual information. Also, poor data quality such as mislabeling, inconsistent annotations, and duplicates can lead to inflated performance and weak generalization. Moreover, by including only the functions, these datasets miss broader program context, like data/control dependencies and interprocedural interactions, that are essential for accurately understanding real-world security flaws. Without this context, detection models are evaluated under unrealistic assumptions. To address these limitations, this paper introduces SecVulEval, a benchmark designed to support fine-grained evaluation of LLMs and other detection methods with rich contextual information. SecVulEval focuses on real-world C/C++ vulnerabilities at the statement level. This granularity enables more precise evaluation of a model's ability to localize vulnerabilities, beyond simple binary classification at the function level. By incorporating rich contextual information, SecVulEval sets a new standard for vulnerability detection benchmarks in realistic scenarios. This benchmark includes 25,440 function samples covering 5,867 unique CVEs in C/C++ projects from 1999 to 2024. We evaluated the SOTA LLMs with a multi-agent-based approach. The evaluation on our dataset shows that the models are still far from accurately predicting vulnerable statements in a given function. The best-performing Claude-3.7-Sonnet model achieves 23.83% F1-score for detecting vulnerable statements with correct reasoning. Finally, we analyze the LLM outputs and provide insights into their behavior in vulnerability detection for C/C++.

==> sec/discussions.tex <==
\section{Failure Analysis}
\song{move this to the appendix}

% \subsection{Failure Analysis}

%\subsubsection{Failed Cases in Vulnerability Detection}

We analyzed our experimental results to shed more light on the behavior of the LLMs on vulnerability detection and repair tasks. 
We identified a few trends that are described below. We made this analysis only on \emph{Qwen2.5-Coder-32B} and \emph{GPT-4.1} models since vulnerabilities detected by other models are too few to make any statistical inference.

Since the models generally struggle to identify the vulnerable lines in a function, we reviewed the functions and vulnerable lines that were correctly detected by the models. We analyzed the functions and the vulnerable lines from various aspects such as size, complexity, etc. Our findings suggest that the models are more likely to correctly identify vulnerable lines from smaller and simpler functions compared to long functions with many conditions and looping. 
%\song{show your results in a figure} \basim{the figure is a bit complicated and cluttered if I put it in one image. so added the figure in Appendix with multiple subfigures.}
While the median size of vulnerable functions in our dataset is 48 lines, the median function sizes where the models correctly identify the vulnerable lines are only 17 and 22 lines for \emph{Qwen2.5-Coder-32B} and \emph{GPT-4o} respectively. This can be visualized in Figure \ref{fig:vul_func_size} in Appendix \ref{appndx:vul_func_size} that the models can identify more vulnerabilities from the smaller functions. Simplicity of the vulnerabilities also helps the models fare better in the detection task. 
Among the vulnerabilities correctly identified by the models, most of them are single-line vulnerabilities, i.e., 76.12\% of them by \emph{Qwen2.5-Coder-32B} and 89.74\% of them by \emph{GPT-4o} are single statement vulnerabilities. This is in sheer contrast to only 31.07\% single-statement vulnerabilities in our full dataset. 

\begin{figure}
    % \newcounter{subfigure}
    \centering
    \begin{minipage}{0.95\linewidth}
        \begin{lstlisting}[style=Cstyle]
int wvlan_set_station_nickname(...){
    // lines skipped due to limited space
    memcpy(lp->StationName, extra, wrqu->data.length);
    // lines skipped due to limited space
}
        \end{lstlisting}
        \vspace{-0.1in}
        \captionof{subfigure}{Correctly identified buffer overflow in line-3}
    \end{minipage}
    \begin{minipage}{0.95\linewidth}
        \begin{lstlisting}[style=Cstyle]
int wvlan_uil_put_info(...){
    // lines skipped due to limited space
    if (...) {
        if (...) {
            switch(...){
            case CFG_CNF_OWN_NAME:  
                memcpy((void *)lp->StationName, (void *)&pLtv->u.u8[2],    (size_t)pLtv->u.u16[0]);
    // lines skipped due to limited space
}
        \end{lstlisting}
        \vspace{-0.1in}
        \captionof{subfigure}{Failed to identify buffer overflow in line-7}
    \end{minipage}
    \caption{\emph{Qwen2.5-Coder-32B} missing similar buffer overflow vulnerability when the vulnerability is inside complex conditionals.}
    \label{fig:disc_code_sample}
\end{figure}

Noting the models' difficulty in identifying multi-line vulnerabilities, we also analyzed their performance based on cyclomatic complexity. 
Particularly, we analyzed how much the models can identify the vulnerabilities that are nested deep within one or more if-else statements or loops. Indeed, our analysis shows that the models are not very good at identifying vulnerabilities that are dependent on other conditionals. 72.85\% vulnerable lines detected by Qwen2.5-Coder-32B are at the function root level (no nesting) and 76.92\% for GPT-4o. On the other hand, the full dataset has only 43.49\% vulnerable lines at the function root level. A Chi-Squared test shows that this is a significant difference between the vulnerable lines in the full dataset and the correctly identified ones (p-value $1.67\mathrm{e}{-06}$ and $5.64\mathrm{e}{-05}$ for Qwen2.5-Coder-32B and GPT-4o, respectively). The two code snippets in Figure \ref{fig:disc_code_sample} show such an instance where Qwen2.5-Coder-32B correctly identified a buffer overflow (CWE-119) vulnerability at the function root level but missed a similar vulnerability that is deeply nested. 
In the \texttt{wvlan\_set\_station\_nickname} function (top snippet, line-3), a string is copied to another memory block using the \texttt{memcpy} function. However, it is possible to cause a buffer overflow with a longer \texttt{lp->StationName} than the \texttt{wrqu->data.length}. The Qwen2.5-Coder-32B model correctly identifies this line but misses the same issue in the \texttt{wvlan\_uil\_put\_info} function (bottom snippet, line-7) which is inside several \texttt{if} and \texttt{switch} statements.

\mybox{Our analysis suggests that current LLMs are primarily capable of detecting vulnerabilities in simple, single statements within relatively small functions.}

%\subsubsection{Failed Cases in Vulnerability Repair}
% Similar to the detection task, we also analyze the vulnerability repair task from the models. 
%For vulnerability repair, we consider instances with low CodeBLEU scores as failures. Our analysis reveals several common factors contributing to these low scores. Notably, we observe a tendency in models, particularly \emph{GPT-4o}, to perform NULL checks. This behavior enables GPT-4o to correctly fix certain instances of CWE-476 (Null Dereference). 
%Almost half of the instances where GPT-4o achieved a full 100\% CodeBLEU score is CWE-476. However, these excessive checks also resulted in a lot of null checks that did not address the actual vulnerability. Often developers maintain implicit rules about certain pointers to be not null and do not need to check every variable for null. These extra null checks reduce the CodeBLEU score for GPT-4o in CWE-476 despite fixing many of them correctly. Another common failure occurs when a vulnerability arises from the absence of a necessary operation rather than a specific faulty line within the function. For example, some instances of CWE-416 (Use-After-Free) stem from missing lock and unlock operations (e.g., \emph{CVE-2017-0861}). In these cases, models must not only detect where locking is missing but also correctly insert it. This added complexity makes repairing such vulnerabilities more challenging for the models. Finally, we also want to mention use cases where the models received low scores due to CodeBLEU's mechanism of evaluation. We share an example in Appendix \ref{appndx:same_code_low_score}, where we show that the model gets a very low score despite giving the correct solution through a different implementation. This highlights the need for a more robust evaluation mechanism. %., particularly for sparse line-level matching in low-context scenarios. 

%\mybox{GPT-4o is inclined towards making excessive null checks which can reduce the scores. Also, all models suffer to repair vulnerabilities that sprout from lack of certain checks instead of vulnerable lines in the function itself.}%\song{add a summarization}\basim{added}

% \song{summarized some patterns regarding the vulnerability repair}

%\subsection{Can Fine-tuning Help?} 

%Fine-tuning has been widely recognized as an effective approach for enhancing the performance of large language models (LLMs)~\cite{ding2023parameter}. 
%To check if the model performance can be improved with appropriate fine-tuning, we perform a simple fine-tuning for line-level vulnerability detection. 
%In this pilot study, we choose CodeLlama due to its open-source accessibility, fine-tuning capabilities, and reproducibility. 
%%performed poorly in our experiments, we check if CodeLlama's performance can be improved and avoid training other models due to resource constraints. 
%We separated 100 random functions (including both vulnerable and non-vulnerable) from our dataset and used the rest of the dataset to train the \emph{CodeLlama-7B-Instruct} model. We used LoRA fine-tuning for three epochs, with $learning\_rate=2\text{e}04$, $lora\_alpha=32$. 
%Lower $r$ values usually only learn output styling and not intricate details, so we choose a higher value $r=16$. 

%Our basic fine-tuning setup has shown impressive performance. On our test data comprising 100 functions, the fine-tuned model recorded a 10\% F1-score, which is 14.4x of what the base \emph{CodeLlama-70B-Instruct} model achieved (0.69\%). We also saw more accurate JSON output, but still not perfect. 
%So, we adopted the same output processing as in our previous experiments. However, there are some caveats to this as well. 
%Due to the training for vulnerability detection, the model was extremely inclined towards predicting vulnerability. In fact, out of our 100 test functions, the fine-tuned model has 86 False Positive predictions, which is significantly high for any practical use. We also faced problems when trying to train with both vulnerable and non-vulnerable functions. 
%Since the non-vulnerable functions do not have any vulnerable lines, the fine-tuning makes the model overfit to non-vulnerable detection, which is why we later fine-tuned with only vulnerable samples. 
%\mybox{Fine-tuning increases CodeLlama’s F1-score by 14.4× but also results in a 94.5\% false positive rate. However, we believe that with more advanced training methods, fine-tuning has the potential to surpass the performance of base models.} 
%\song{Previously, you have fine-tuned codellama, please also discuss the potential and issues of fine-tuning codellama on vulnerability detection}
% \begin{figure}[t]
%     % \refstepcounter{listing}
%     \begin{subfigure}[]{\linewidth}
%     \centering
%     \begin{lstlisting}[style=Cstyle]
% int wvlan_set_station_nickname(...){
%     // lines skipped due to limited space
%     memcpy(lp->StationName, extra, wrqu->data.length);
%     // lines skipped due to limited space
% }
%     \end{lstlisting}
%     \caption{Some caption.}
%     \label{lst:codeblockA}            
%     \end{subfigure}%
    

%     \begin{lstlisting}[style=Cstyle]
% int wvlan_uil_put_info(...){
%     // lines skipped due to limited space
%     if (...) {
%         if (...) {
%             switch(...){
%             case CFG_CNF_OWN_NAME:  
%                 memcpy((void *)lp->StationName, (void *)&pLtv->u.u8[2],    (size_t)pLtv->u.u16[0]);
%     // lines skipped due to limited space
% }
%     \end{lstlisting}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}
%Most of the previous benchmarks on C/C++ vulnerabilities focus on binary classification at file or function level, and does not incorporate line-level vulnerability labeling. There are metrics such as F1-score to accurately represent such binary outcomes. However, in case of line-level vulnerability, the same is not necessarily true. When matching vulnerable line predictions with the reference, the prediction will not pass if a single line mismatch is found. But in practice, a correct vulnerable lines detection with 1-2 lines before/after can still be useful to a developer compared to scouring the whole function in search of the vulnerable lines. Therefore, an evaluation metrics that can capture this information along with syntactical and semantic similarity can be useful, particularly for test-less projects like Linux.

==> sec/limitation.tex <==
\section{Limitation}
\basim{Limitation section is required for NeurIPS}
While \textsc{SecVulEval} makes a significant step forward for Linux vulnerability research, there are some aspects that should be considered with our findings.

% \basim{kindly check if the internal/external classification is appropriate.}
\textit{Internal threats:} Output parsing failure is a common problem faced by researchers when working with LLMs because of their random behavior. This can affect the results as some LLM outputs might be excluded from analysis due to parsing errors. We mitigated this issue by explicitly prompting the models to output in json formats, along with few-shot examples. Moreover, we added an output post-processing stage to further reduce the error. Another source of threat is the prompts used for the study. LLMs' outputs can be strongly correlated with the input prompt. We kept a similar prompt with the same randomly selected few-shot examples across all models for fair comparisons, with slightly adjusting to specific model behaviors.

\textit{External threats:} NVD is a popular and long-standing source for vulnerability curation and it is possible that the models may have been pre-trained on specific vulnerability data. This may not accurately present the models' performances on future unseen data. Another potential discrepancy in models can arise from the implementation of the models. To mitigate this, we used all the models from HuggingFace\footnote{https://huggingface.co} using the \emph{transformers.pipeline} implementation, and official model generation examples from the HuggingFace model homepage. We left most of the hyperparameters to default settings as they have been thoroughly evaluated by the community and is standard.

==> sec/quantitative.tex <==
\section{Quantitative Analysis}

==> sec/reference.tex <==
\section*{References}


References follow the acknowledgments in the camera-ready paper. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
Note that the Reference section does not count towards the page limit.
\medskip


{
\small


[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.


[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.


[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.
}

